Reducing Hallucinations in Vision-Language Models via Latent Space Steering

Hallucination poses a challenge to the deployment of large vision-language models (LVLMs) in applications. Unlike in large language models (LLMs), hallucination in LVLMs often arises from misalignments between visual inputs and textual outputs. This paper investigates the underlying mechanisms of hallucination, focusing on the unique structure of LVLMs that distinguishes them from large language models (LLMs). We identify that hallucinations often arise from the sensitivity of text decoders to vision inputs, a natural phenomenon when image encoders and text decoders are pre-trained separately. Inspired by this, we introduce Visual and Textual Intervention (VTI), a novel technique designed to reduce hallucinations by steering latent space representations during inference to enhance the stability of vision features. As a task-agnostic test-time intervention, VTI can be easily applied to any problem without additional cost. Extensive experiments demonstrate that it can effectively reduce hallucinations and outperform baseline methods across multiple metrics, highlighting the critical role of vision feature stability in LVLMs.

==> sections/backgrounds.tex <==
\section{Backgrounds}
\label{sec:backgrounds}
\paragraph{In-context learning}
In the setting of in-context learning, consider the task of transferring negative sentiment to positive sentiment. A prompt is constructed by concatenating independent demonstration examples $X_{demos}$, e.g. ``\{1 star, I hate it!\} is rewritten as \{5 stars, I love it!\}'' followed by a query example: ``\{I don't like the t-shirt\} is rewritten as \{''. Specifically, in-context learning assumes a target task with
demonstration data $X_{demos} = \{(x_i
, y_i)|\, i = 1,\dots,k\}$. To perform the task for a given query example $x_{q}$, the model is asked to predict $y_{q}$ based on the demonstrations. In traditional settings, $y$ is often a single word that represents the categorical label. However, $y$ could potentially be a sentence or paragraph that is related to $x$. For example, $y$ can be an adapted version of $x$ in another tone or a paraphrase of $x$ following a specific style. 
\vspace{-3mm}
\paragraph{In-context learning as latent feature shifting} 
\label{sec:featureshifting}
Large language models adopt Transformer~\cite{vaswani2017attention} as the backbone architecture. As a crucial component of the Transformer, self-attention layers relate different positions of a single sequence to compute a representation of the same sequence. Let $X = \text{Concate}\left([X_{demos}, X_{query}]\right)$ denote the inputs (including demonstrations $X_{demos}$ and the query examples $X_{query}$) for a specific self-attention layer of the Transformer. Let $W_k, W_q, W_v$ be the learnable key, query, and value matrix in that layer. In the in-context learning setting, the prefixed demonstration examples simply change the attention module through
prepending a context matrix before the original query example. When the demonstrations $X_{demos}$ are provided as the context, the attention layer for each token $x_{query}$ in the query example $X_{query}$ can be formulated as:
\vspace{-2mm}
\begin{align*}
    &\text{Attn}(x_{query}W_{q},X W_k, X W_v)
%     =& \text{Attn}(x_{query}W_q, [X_{demos}, X_{query}]W_k, [X_{demos}, X_{query}]W_v)\\
%     =&\text{softmax}\left(x_{query}W_q\begin{pmatrix}
% X_{demos}\\ X_{query}
% \end{pmatrix}W_k\right)\begin{pmatrix}
%  X_{demos} \\
% X_{query}
% \end{pmatrix}W_v\\
%  =& \alpha \text{Attn}(x_{query}W_q,X_{query}W_k,X_{query}W_v)\\ 
% & \quad + (1-\alpha)\text{Attn}(x_{query}W_q,X_{demos}W_k,X_{demos}W_v)\\
 =: \alpha h(X_{query}) + (1 - \alpha) h(X_{demos}),
\end{align*}
where $\alpha$ is a scalar that represents the sum of normalized attention weights between demonstrations and query examples (See details in the Appendix~\ref{sec:appendix_fs}). Note that the first term, $h(X_{query})$, is the original attention output without demonstration examples, whereas the second term is a position-wise modification that is based on demonstrations.  Therefore, in-context learning essentially applies a position-wise modification to the original attention output $h$ by shifting the original output feature. The direction of the shift and the distance of the shift are automatically controlled by the self-attention mechanism. 
% \james{The connection between the last sentence and the equation is not clear; explicitly explain what $h$ and $\Delta h$ represents.} 

